Level the Level: Balancing Game Levels for Asymmetric Player Archetypes With Reinforcement Learning

Balancing games, especially those with asymmetric multiplayer content, requires significant manual effort and extensive human playtesting during development. For this reason, this work focuses on generating balanced levels tailored to asymmetric player archetypes, where the disparity in abilities is balanced entirely through the level design. For instance, while one archetype may have an advantage over another, both should have an equal chance of winning. We therefore conceptualize game balancing as a procedural content generation problem and build on and extend a recently introduced method that uses reinforcement learning to balance tile-based game levels. We evaluate the method on four different player archetypes and demonstrate its ability to balance a larger proportion of levels compared to two baseline approaches. Furthermore, our results indicate that as the disparity between player archetypes increases, the required number of training steps grows, while the model's accuracy in achieving balance decreases.

==> content/buffer.tex <==

\section{Introduction}

Game levels for competitive play must be balanced in order to ensure player satisfaction and to avoid frustration or boredom~\cite{becker_what_2020}. The process of balancing a game, however, involves a lot of manual work, effort, and human play testing~\cite{schreiber_game_2021}. For this reason, many works propose approaches to automate the process of game balancing~\cite{beau_automated_2016,volz_demonstrating_2016,pfau_dungeons_2020,morosan_automated_2017,lanzi_evolving_2014,lara-cabrera_balance_2014}. 

Well-designed games ensure the viability of multiple strategies for players to choose from, all of which, if played well, can lead to winning the game~\cite{schreiber_game_2021}.
As a result, many modern games make use of asymmetric balancing strategies, such as pitting heroes of different abilities against each other. This can be seen in dungeon crawlers like \emph{Decent: Journeys in the Dark} or MOBA (Multiplayer Online Battle Arena) games like \emph{League of Legends}. Asymmetric balance there is mainly achieved by balancing the numerical values of game entities, such as health or attack values. Limited work~\cite{beau_automated_2016,lanzi_evolving_2014}, however, has been published to balance games for asymmetric games, i.e. players with different abilities and stats. 
For this reason, this work focuses on ensuring the balance for asymmetric players entirely through \emph{level design}, e.g., where to place resources in relation to the players' spawn positions, framing this task as a procedural content generation (PCG) problem. 
Furthermore, this allows the approach to be used in additional settings, such as when players of different skill levels face each other, such as experts and beginners, or adults playing against children. Another use case is to ensure balance in competitive settings where players with different gear levels are of different strength.

Recently, the Procedural Content Generation via Reinforcement Learning framework (PCGRL) has shown promising results in creating tile based levels~\cite{khalifa_pcgrl_2020}. It has been further extended to apply it to game balancing~\cite{rupp_balancing_2023,rupp_simulation_2024}, where the balance of a level is determined through multiple simulations using heuristic agents. A levels is considered balanced when all players win equally often. An additional survey concludes that the automated balancing simulated through artificial agents actually improves the balance for humans in most cases~\cite{rupp_might_balanced_2024}.

This approach is, however, limited by the fact that it only uses  exactly the same type of agents playing against each other. To address this shortcoming, this work extends the previous research by adding three new types of agents to investigate the ability of the method to achieve balance for agents of different types playing against each other.
We evaluate and compare our results to an additional hill climbing  and the original PCGRL approach. In addition, we introduce an improved version of the action space introduced in~\cite{rupp_balancing_2023} that halves the size of the action space for faster convergence in training.
The code of the introduced heuristic agents and the game environment can be found on Github\footnote{The link to Github is anonymized for double-blind review.}.
Our contributions are:
\begin{itemize}
    \item The asymmetric balancing of game levels with reinforcement learning on the example of various different heuristic player types.
    \item An improvement in the definition of the action space for the Markov Decision process that halves the size of the action space resulting in faster convergence in training.
    \item A detailed study to evaluate the results against a hill climbing approach and also in comparison to the original PCGRL method.
    %\item A re implementation of the game environment used in~\cite{rupp_balancing_2023} to speed up simulations and additional heuristic agents.
\end{itemize}


\section{Related Work}
There are several approaches to balancing a game, one of which is to configure the values of certain game entities~\cite{schreiber_game_2021}.
For asymmetric games, Beau et al.~\cite{beau_automated_2016} propose an approach using Monte Carlo simulations for estimating the impact of game actions and demonstrate how to find imbalances in the value configuration. Like this work, they then also balance imbalances until they are balanced according to the approximation through simulations. Evolutionary algorithms have been used by Volz et al..~\cite{volz_demonstrating_2016} to the balancing and deck building for card games, by De Mesentier Silva~\cite{mesentier_silva_evolving_2019} to balance the meta of a collectible card game, and by Morosan et al.~\cite{morosan_automated_2017} for real time strategy (RTS) games. Whereas Pfau et al. optimize game parameters using data-driven deep player behavior models.

In contrast, this work focuses on the automated balancing of games through the level design entirely using PCG. Lanzi et al.~\cite{lanzi_evolving_2014} introduced an evolutionary algorithm for balancing maps for first person shooters. The authors also include the balancing of asymmetries by using bots each with different weapon types. Lara Cabrera et al.~\cite{lara-cabrera_balance_2014} balance game maps for an RTS game also using an evolutionary algorithm.
This work builds upon and extends the work by Rupp et al.~\cite{rupp_balancing_2023,rupp_simulation_2024} where RL is introduced to balance tile-based levels. A more detailed explanation for better understanding is given in the background chapter (Section~\ref{sec:pcg-balancing}).

Besides game balancing, PCG is an active field of research to generate game related content such as game levels in general~\cite{togelius_search-based_2011,khalifa_pcgrl_2020}, rules~\cite{cook_mechanic_2013}, quests~\cite{ashby_personalized_2023}, or narratives~\cite{alvarez_tropetwist_2022}.


\section{Background}

\subsection{PCGRL for Game Level Balancing}
\label{sec:pcg-balancing}
Khalifa et al. introduced the PCGRL framework~\cite{khalifa_pcgrl_2020} to model level generation as a Markov decision process, leveraging reinforcement learning (RL). Within this iterative process, the RL agent receives rewards for modifying the current state until the level meets predefined constraints expressed through the reward function. 

Based on this approach, Rupp et al. introduced an approach using PCGRL to balance previously generated levels~\cite{rupp_balancing_2023,rupp_simulation_2024}. Thereby, the balancing is considered as a fine-tuning process for existing levels which has shown to converge faster compared to when generating and balancing levels in one step.
For balancing, only tile swaps are used as modifications. Rewards are computed by conducting multiple simulations, wherein two identical heuristic agents are playing the game. The reward is determined by the frequency of each agent's victory in the game and can be understood as a static simulation-based evaluation function as defined in~\cite{yannakakis_experience-driven_2011}. This function assigns a value to each level that represents the balance in $[0,1]$, where 0.5 indicates equal win rates for both players, 0 and 1 indicate that a particular player wins each round.

In contrast to search-based approaches, RL can generate content fast once the model is trained. In particular, this is important here as the simulations used in the reward step are computationally expensive. As RL learns throughout training, unnecessary simulation steps are learned to be avoided which speeds up the inference. For all PCGRL approaches Proximal Policy Optimization (PPO)~\cite{schulman_proximal_2017} is applied as RL algorithm.

An additional survey including human playtesters concludes that the balancing simulated with artificial heuristic agents actually improves the perceived balance for humans in most cases~\cite{rupp_might_balanced_2024}.


\subsection{Game Environment}
The game is a survival challenge on a 6x6 tile-based map set within the Neural Massively Multiplayer Online (NMMO)
environment~\cite{suarez_neural_2019} where two players compete for food and water resources. Victory is achieved by either collecting five food resources or by %outlasting
surviving the opponent. There are four tile types: grass~\raisebox{-0.2em}{\includegraphics[width=1em]{content/img/tiles/Grass.png}}, rock~\raisebox{-0.2em}{\includegraphics[width=1em]{content/img/tiles/Wall.png}}, water~\raisebox{-0.2em}{\includegraphics[width=1em]{content/img/tiles/Water.png}}, and food~\raisebox{-0.2em}{\includegraphics[width=1em]{content/img/tiles/Forest.png}}. Rock and water tiles impede movement.

Players make moves simultaneously, choosing from four directions: up, down, left, or right. Like in NMMO, their states include position, health, water, and food levels. Each turn, players lose water and food, with health depleting if both reach zero. When a player's health indicator reaches zero, the player has lost. Players can replenish food by consuming food tiles, which then become scrub tiles. There's a 2.5\% chance for scrub tiles to respawn as food. Water can be replenished by moving onto adjacent water tiles, which are never depleted. Health is restored gradually if food and water levels exceed 50\%.
The red player~\raisebox{-0.2em}{\includegraphics[width=1em]{content/img/tiles/Player_Tile.png}} is player one and the yellow player~\raisebox{-0.2em}{\includegraphics[width=1em]{content/img/tiles/Opponent_Tile.png}} is player two. In this work, both players are controlled by heuristic agents based on a greedy strategy, always collecting the nearest available food resource (Algorithm~\ref{alg:forage-agent}). For the experiments, this heuristic will be slightly modified to create several different heuristic agent types (cf. Section~\ref{sec:a-balancing}).

\section{Method}

\subsection{Improving the action space}

For this work, we use the \emph{swap-wide} representation as definition of the action space of the Markov Decision process for balancing as it achieves the best results in~\cite{rupp_simulation_2024}. This action space enables the RL agent to swap the tile of a predicted location $(x1,y1)$ with the tile of a second predicted location $(x2,y2)$ of a level. With another flag it can predict if the swap should be implemented or not. This results in an action space dependent on the height $h$ and width $w$ of the level: $[h,w,h,w,2]$. For a 6x6 level this results in 2592 actions.

Since the model already does a prediction on the position where to swap tiles, the additional prediction wether to swap or not makes the action space unnecessary complex. Therefore we propose to only predict the two swapping positions resulting in the action space: $[h,w,h,w]$. For a 6x6 level this reduces the action space to the half of 1296 actions.

\subsection{Asymmetric Balancing}
\label{sec:a-balancing}

In this work, we introduce the three new agent types B, C, and D, which are derived from the existing agent type A (Algorithm~\ref{alg:forage-agent}).
Agents are implemented by a \textsc{step} function, which is called once per turn for each agent. The step function always returns one of the five actions, describing which of the four adjacent tiles to move to next, or to do nothing. The helper functions \textsc{foodReachable} and \textsc{waterReachable} use path finding if there is a valid path from the agent's position to at least one of the respective resources. If so, the A* algorithm is used to find the shortest path, always favoring food resources as they have a greater impact on winning the game.


\begin{algorithm}
\caption{Heuristic Agent Type A as used in~\cite{rupp_balancing_2023,rupp_simulation_2024}.}
\label{alg:forage-agent}
\begin{algorithmic}[1]

\Procedure{Step}{gameState}
    \State \textbf{initialize} \textit{action} $\leftarrow$ \textbf{DoNotMove}
    \State \textbf{initialize} \textit{foodReachable} $\leftarrow$ \Call{foodReachable}{gameState}
    \State \textbf{initialize} \textit{waterReachable} $\leftarrow$ \Call{waterReachable}{gameState}
    
    \If{foodReachable}
        \State \textit{action} $\leftarrow$
        \Call{findShortestPathTo}{food}
    \ElsIf{waterReachable}
        \State \textit{action} $\leftarrow$
        \Call{findShortestPathTo}{water}
    \EndIf
    \State \Return action
\EndProcedure
\end{algorithmic}
\end{algorithm}


\noindent Each new type of agent addresses a specific aspect of the balance such as movement advantages or scoring victory points by consuming food. The list below gives a brief description of the agents used and how this affects their chance of victory in compared to agent A.
\begin{itemize}
    \item Type A, the "Forage Agent", as described in Algorithm~\ref{alg:forage-agent} and applied in~\cite{rupp_balancing_2023,rupp_simulation_2024}.
    \item Type B, the "Mountain Agent", can also move over mountain tiles and is only blocked by water tiles. This gives it an advantage over type A agents.
    \item Type C, the "Handicap Agent", agent can only perform an action every second turn. This agent is at a huge disadvantage when playing against type A agents.
    \item Type D, the "Double Food Agent", already wins the game with four (D1) or three (D2) collected food resources instead of five. This gives it an advantage over type A agents.
\end{itemize}


% new agents definition

\section{Results, Discussion and Limitations}

For all experiments we use the same dataset of 500 generated levels to ensure a fair comparison. We compare our PCGRL method with to baselines: a random agent and a simple hill climbing approach as used in~\cite{rupp_simulation_2024}. The hill climbing approach applies the same swapping mechanism, however chooses the positions randomly. If the reward is not positive it transitions back to the previous state.
A key metric for evaluation is the proportion of how many levels a method can balance.

For the experiments we train several models where agent type A faces the new agent types in a 1v1 setting. For all PPO models we use two 3-layered multi-layer perceptrons with layers in the sizes 64, 128, and 64 as feature extractor and for the value function. Each model is trained at least for 14 million steps which results in 456 updates of the policy. We use a step size of 512 and parallelize 60 environments. This results in 30.720 trajectories for updating the policy and the neuronal networks per single update.


To assess the imbalance of a specific agent setup, we calculate the proportion of dataset levels initially skewed towards that agent, where the agent wins more often in simulations than its opponent. Initially balanced levels are not considered. Figure~\ref{fig:unfairness} shows the relation of the initial unfairness and the amount of training steps needed for convergence.
%When inspecting the initial balance for the different agent settings in the level dataset, we see larger proportions balanced towards a specific player. 
If both agent types are identical, the proportion of levels initially balanced to one distinct player are even (0.5). 
In contrast, for the setup of A vs. B 68.9\%, A vs. C 85.8\%, and A vs. D1 61.4\%, A vs. D2 78.5\% are heavily unbalanced towards a specific player.
Comparing the initial unfairness with the number of training steps required for model convergence reveals that the greater the initial unfairness of a setup, the more training steps are needed.
%From this we conclude that type B and D have an advantage over type A based on the agent's skills, and that type C has a strong disadvantage over type A. This is in line with our previous intention regarding the design of the agents.

% A vs. B 27\%, A vs. C 88\%, and A vs. D 19\% 

\begin{table}
    \centering
    \caption{Comparison of the proportions of balanced levels on a set of 500 generated levels with two baselines approaches.}
    \begin{tabular}{ccccc} \toprule
           \textbf{Agents}&  \textbf{Random (\%)} & \textbf{Hill Climbing (\%)} & \textbf{PCGRL (\%)} \\
    \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5}           
        A vs. B &  27.6 &  46.1  & \textbf{80.8} \\
        A vs. C &  16.2 &  24.6 & \textbf{58.2} \\
        A vs. D1 &  28.8 &  46.6 & \textbf{73.4} \\ 
        A vs. D2 &  26.8 &  35.2 & \textbf{59.2} \\ \midrule
        A vs. A~\cite{rupp_simulation_2024} &  - &  59.6 & 68.0 \\ \bottomrule
    \end{tabular}
    \label{tab:symmetries}
\end{table}



\subsection{Performance and Comparison to Baselines}

\subsection{Generated Levels}



\section{Conclusion}
